Ring-a-Pose: A Ring for Continuous Hand Pose Tracking

We present Ring-a-Pose, a single untethered ring that tracks continuous 3D hand poses. Located in the center of the hand, the ring emits an inaudible acoustic signal that each hand pose reflects differently. Ring-a-Pose imposes minimal obtrusions on the hand, unlike multi-ring or glove systems. It is not affected by the choice of clothing that may cover wrist-worn systems. In a series of three user studies with a total of 30 participants, we evaluate Ring-a-Pose's performance on pose tracking and micro-finger gesture recognition. Without collecting any training data from a user, Ring-a-Pose tracks continuous hand poses with a joint error of 14.1mm. The joint error decreases to 10.3mm for fine-tuned user-dependent models. Ring-a-Pose recognizes 7-class micro-gestures with a 90.60% and 99.27% accuracy for user-independent and user-dependent models, respectively. Furthermore, the ring exhibits promising performance when worn on any finger. Ring-a-Pose enables the future of smart rings to track and recognize hand poses using relatively low-power acoustic sensing.

==> aug-results.tex <==
\begin{table}[t]
    \caption{Data Augmentation and Input Normalization Ablation Study Results. ``UD'' stands for user dependence, and ``UI'' stands for user independence. All errors refer to mean per-joint position error (MPJPE).}
    \centering
    \begin{tabular}{|c|>{\centering\arraybackslash}m{2cm}|>{\centering\arraybackslash}m{2cm}|>{\centering\arraybackslash}m{2cm}|>{\centering\arraybackslash}m{2cm}|}
        \hline
         & \begin{tabular}[c]{@{}c@{}}UI \\ Training\end{tabular}  &  \begin{tabular}[c]{@{}c@{}}UD \\ Training\end{tabular}& \begin{tabular}[c]{@{}c@{}}UI \\ Robustness\end{tabular} & \begin{tabular}[c]{@{}c@{}}UD \\ Robustness\end{tabular} \\
         \hline
         w/o data augmentation& 14.16 & 10.67 & 15.24 & 12.92 \\
         \hline
         w/o vertical shifts&  14.37 & 10.62 & 15.25 & 12.94 \\
         \hline
         w/o randomness& 14.07 & 10.48 & 14.76 &  12.68\\
         \hline
         w/o input norm& 14.34 & 10.43 & 15.06 & 12.63\\
        \hline
         \begin{tabular}[c]{@{}c@{}}w/ data augmentation\\ w/ input norm\end{tabular}&  14.12& 10.44 & 14.74 & 12.70\\
         \hline
    \end{tabular}
    \label{tab:my_label}
\end{table}


==> gesture-results.tex <==

\begin{table}[t]
    \centering
    \caption{Hand gesture recognition performance comparison. ``SD'' stands for session dependence, ``UD'' stands for user dependence, and ``UI'' stands for user independence.}
    \begin{tabular}{|c|c|S[table-format=2.2, table-column-width=1.7cm]|S[table-format=2.2, table-column-width=1.7cm]|S[table-format=2.2, table-column-width=1.7cm]|}
    \hline
        System & Gesture Set & {SD Accuracy} & {UD Accuracy} & {UI Accuracy}\\
    \hline
        CyclopsRing, 2015~\cite{Cyclopsring} & 7 gestures & \textemdash & \textemdash & 84.75\%\\
    \hline
        FingerPing, 2018~\cite{FingerPing} & 10 gestures & 95.64\% & \textemdash & \textemdash\\
    \hline
        PeriSense, 2020~\cite{PeriSense} & 8 gestures & \textemdash & 98\% & \textemdash\\
    \hline
        \textbf{\theDevice{}} & 9 gestures & \textemdash & 97.03\% & 72.54\%\\
    \hline
    \end{tabular}
    \label{table:gest-results}
\end{table}
